Graph Pruning for Enumeration of Minimal Unsatisfiable Subsets

Finding Minimal Unsatisfiable Subsets (MUSes) of binary constraints is a common problem in infeasibility analysis of over-constrained systems. However, because of the exponential search space of the problem, enumerating MUSes is extremely time-consuming in real applications. In this work, we propose to prune formulas using a learned model to speed up MUS enumeration. We represent formulas as graphs and then develop a graph-based learning model to predict which part of the formula should be pruned. Importantly, our algorithm does not require data labeling by only checking the satisfiability of pruned formulas. It does not even require training data from the target application because it extrapolates to data with different distributions. In our experiments we combine our algorithm with existing MUS enumerators and validate its effectiveness in multiple benchmarks including a set of real-world problems outside our training distribution. The experiment results show that our method significantly accelerates MUS enumeration on average on these benchmark problems.

==> algorithms/graph_prune.tex <==
\begin{algorithm}
    \caption{Prune a Graph with node labels}\label{alg:graph_prune}
    \textbf{Input} $G(V,E)$, $\by$\\
    \textbf{Output} $G'(V',E')$\\
    \begin{algorithmic}[1]
        \Require $\by \in \{0,1\}^{|V|}$
        \State $V' \gets V$ \Comment{Initialize pruned node set}
        \State $E' \gets E$ \Comment{Initialize pruned edge set}
        \State $M \gets |V|$
        \While {$i<M$}
        \If {$y_i=0$}
        \State $V' \gets V' \backslash \{v_i\}$ \Comment{Remove node}
        \State $E'\gets E' \backslash \{(u,w)  | u,w \in V, u=v_i or w=v_i\}$
        \EndIf
        \State i $\gets i+1$
        \EndWhile\\
        \Return $G'(V',E')$
    \end{algorithmic}
\end{algorithm}

==> algorithms/greedy_prune.tex <==
\begin{algorithm}[t]
    \caption{Greedily prune a CNF formula}\label{alg:greedy_prune}
    \textbf{Input} $\formula=(U,C)$, $\bmu$, k\\
    \textbf{Output} $\formula'=(U',C')$\\
    \begin{algorithmic}[1]
        %\Require $\bmu \in R^{|C|}$, $k \in \bbN$
        \State $step \gets \frac{max(\bmu)}{k}$
        \State $t \gets step$
        %\State $threshold \gets max(\by) - step$
        \State $\by \gets \bmu \le t$ \Comment{aggressively pruning initially}
        \State $\formula' \gets Prune(\formula,\by)$ \Comment{using eq. \ref{eq:prune}}
        \While{$SAT(\formula')$}
        \State $t \gets t + step$
        \State $\by \gets \bmu\le t$
        \State $\formula' \gets Prune(\formula,\by)$
        \EndWhile\\
        \Return $\formula'$
    \end{algorithmic}
\end{algorithm}


==> algorithms/prune.tex <==
\begin{algorithm}
    \caption{Prune a CNF formula}\label{alg:prune}
    \textbf{Input} $\formula$, $\by$\\
    \textbf{Output} $\formula'$\\
    \begin{algorithmic}[1]
        \Require $\by \in \{0,1\}^{|C|}$
        \State $C' \gets C$ \Comment{Initialize pruned clause set}
        \State $M \gets |C|$
        \While {$i<M$}
        \If {$y_i=0$}
        \State $C' \gets C' \backslash \{c_i\}$ \Comment{Remove clause}
        \EndIf
        \State i $\gets i+1$
        \EndWhile
        \State $U' \gets \{u_i | c_i \in C'\}$ \Comment{Remove unused variables}\\
        \Return $\formula'$
    \end{algorithmic}
\end{algorithm}

==> figures/graph_color.tex <==
\begin{figure*}[h]
  \centering
  \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{photos/graph_color.png}
      \caption{Initial graph}
      \label{fig:gc_full}
    \end{subfigure}\hspace*{-0.5cm}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{photos/graph_color_scores.png}
      \caption{Pruning score visualization}
      \label{fig:gc_scores}
    \end{subfigure}\hspace*{-0.5cm}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[width=1\linewidth]{photos/pruned_graph_color.png}
      \caption{Post-pruning Graph}
      \label{fig:gc_pruned}
    \end{subfigure}

  \caption{The initial graph in (a) along with the coloring number $K=4$ is translated into CNF and the resulting formula is pruned. (b) shows the average pruning probability for clauses associated with each node. The pruned formula is then converted back into the graph (c) for plotting. Dashed edges are relaxed, allowing neighboring nodes to share colors. The post-prunning graph has many relaxed edges, as its corresponding CNF formula has fewer constraints.}
  \label{fig:graph_color}
\end{figure*}

==> figures/graph_color_combined.tex <==
\begin{figure*}[h]
    \centering
   
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{photos/wheel_graph_color.png}
        %\caption{Initial graph}]
      \end{subfigure}\hspace*{-0.5cm}
      \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{photos/wheel_graph_color_scores.png}
        %\caption{Pruning score visualization}
      \end{subfigure}\hspace*{-0.5cm}
      \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{photos/pruned_wheel_graph_color.png}
       % \caption{Post-pruning Graph}
      \end{subfigure}
      
      \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{photos/graph_color.png}
        \caption{Initial graph}
        \label{fig:gc_full}
      \end{subfigure}\hspace*{-0.5cm}
      \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{photos/graph_color_scores.png}
        \caption{Pruning score visualization}
        \label{fig:gc_scores}
      \end{subfigure}\hspace*{-0.5cm}
      \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{photos/pruned_graph_color.png}
        \caption{Post-pruning Graph}
        \label{fig:gc_pruned}
      \end{subfigure}
    
    \caption{The initial graphs in (a) along with the coloring number $K=4$ are translated into CNF and the resulting formulas are pruned. (b) shows the average pruning score for clauses associated with each node, with lighter colors indicating higher pruning confidence. The pruned formulas are then converted back into graphs (c) for plotting.  Dashed edges are relaxed, allowing neighboring nodes to share colors. The examples demonstrate two different strategies the model can use to prune graph coloring problems. In the sparser graph, completely removing the central node shrinks the formula significantly. In the denser graph, the model instead relaxes many edges, allowing neighboring nodes to share colors. Both approaches yield unsatisfiable formulas with fewer constraints which can accelerate MUS enumeration.}
    \label{fig:graph_color}
\end{figure*}

==> figures/wheel_graph_color.tex <==
\begin{figure*}[h]
    \centering
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{photos/wheel_graph_color.png}
        \caption{Initial graph}
        \label{fig:gc_full}
      \end{subfigure}\hspace*{-0.5cm}
      \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{photos/wheel_graph_color_scores.png}
        \caption{Pruning score visualization}
        \label{fig:gc_scores}
      \end{subfigure}\hspace*{-0.5cm}
      \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{photos/pruned_wheel_graph_color.png}
        \caption{Post-pruning Graph}
        \label{fig:gc_pruned}
      \end{subfigure}

    \caption{The initial graph in (a) along with the coloring number $K=4$ is translated into CNF and the resulting formula is pruned. (b) shows the average pruning score for clauses associated with each node. The pruned formula is then converted back into the graph (c) for plotting.  Dashed edges are relaxed, allowing neighboring nodes to share colors. The post-prunning graph is smaller but maintains many non 4-colorable subgraphs, lending itself to easier MUS enumeration.}
    \label{fig:graph_color}
\end{figure*}

==> tables/extrap_enum.tex <==
\begin{table*}[h]
    \footnotesize
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Solver}    & \textbf{100 vars.}          & \textbf{150 vars.}          & \textbf{200 vars.}         & \textbf{250 vars.}         & \textbf{300 vars.}        \\
        \hline
        MARCO              & 1145.92$\pm$ 36.0           & 348.56$\pm$ 17.84           & 103.0$\pm$ 8.13            & 55.6$\pm$ 7.52             & 19.33$\pm$ 3.31           \\
        GRAPE-MUST + MARCO & \textbf{1157.69$\pm$ 34.03} & \textbf{357.43$\pm$ 17.98}  & \textbf{108.21$\pm$ 8.47}  & \textbf{60.31$\pm$ 8.7}    & \textbf{20.25$\pm$ 3.31}  \\
        \hline
        Remus              & 5188.03$\pm$ 149.6          & 1493.73$\pm$ 77.36          & 404.66$\pm$ 35.97          & 156.41$\pm$ 19.74          & 63.29$\pm$ 14.78          \\
        GRAPE-MUST + REMUS & \textbf{1157.69$\pm$ 34.03} & \textbf{2216.71$\pm$ 91.92} & \textbf{630.75$\pm$ 50.52} & \textbf{220.49$\pm$ 25.72} & \textbf{66.38$\pm$ 11.69} \\
        \hline
        Tome               & 723.29$\pm$ 23.32           & 218.99$\pm$ 9.81            & 68.02$\pm$ 4.56            & 30.31$\pm$ 3.03            & 11.13$\pm$ 1.75           \\
        GRAPE-MUST + TOME  & \textbf{848.8$\pm$ 27.96}   & \textbf{244.87$\pm$ 11.11}  & \textbf{76.67$\pm$ 5.03}   & \textbf{35.56$\pm$ 3.42}   & \textbf{12.86$\pm$ 2.02}  \\
        \hline
    \end{tabular}
    \caption{Enumeration results from the extrapolation experiment.}
    \label{tab:extrap_enumeration}
\end{table*}

==> tables/extrap_prune.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \textbf{\# Variables}    & \textbf{Pruning \%}         \\            
        \hline
        100           &    30.22\% $\pm$ 0.83\%       \\
        \hline
        150             & 29.16\% $\pm$ 1.14\%          \\
        \hline
        200     & 27.68\% $\pm$ 1.26\% \\
        \hline
        250     & 24.28\% $\pm$ 1.45\% \\
        \hline
        300     & 23.48\% $\pm$ 1.48\%\\
        \hline
    \end{tabular}
    \caption{Average percentage of the original formula pruned by GRAPE-MUST. }
    \label{tab:extrap_reductions}
\end{table}

==> tables/longer_timeout.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Solver (30 mins.)} & \textbf{Random Problems} & \textbf{Logistics Planning} & \textbf{Graph Coloring}  \\ \hline
        Marco                      & $96220 \pm 7129$         & $172933.72 \pm 16285.18$    & $128638.94 \pm 23702.68$ \\
        GRAPE-MUST + Marco         & $97254 \pm 6822$         & $177356.60 \pm 16373.36$    & $176703.96 \pm 31061.28$ \\ \hline
        Remus                      & $484033 \pm 25554$       & $82774.54 \pm 5690.20$      & $8965.48 \pm 1121.03$    \\
        GRAPE-MUST + Remus         & $504056 \pm 28010$       & $87825.64 \pm 6239.49$      & $15525.12 \pm 3201.24$   \\ \hline
        Tome                       & $73644 \pm 3318$         & $24403.12 \pm 2843.69$      & $72476.06 \pm 16174.54$  \\
        GRAPE-MUST + Tome          & $73442 \pm 3719$         & $25903.40 \pm 2842.90$      & $54981.82 \pm 12340.48$  \\ \hline
    \end{tabular}
    \caption{Average number of MUSes found by each solver in 30 minutes.}
    \label{tab:longer_timeout}
\end{table*}

==> tables/reductions.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \textbf{Problem}    & \textbf{Pruning \%}                     \\
        \hline
        Random Formulas            &    32.22\% $\pm$ 0.83\%       \\
        \hline
        Logistics Planning              & 36.27\% $\pm$ 1.56\%          \\
        \hline
        Graph Coloring(4-7)     & 30.18\% $\pm$ 1.00\% \\
        \hline
    \end{tabular}
    \caption{Average percentage of the original formula pruned by GRAPE-MUST. }
    \label{tab:reductions}
\end{table}
